Achieving Energetic Superiority Through System-Level Quantum Circuit Simulation

Quantum Computational Superiority boasts rapid computation and high energy efficiency. Despite recent advances in classical algorithms aimed at refuting the milestone claim of Google's sycamore, challenges remain in generating uncorrelated samples of random quantum circuits. In this paper, we present a groundbreaking large-scale system technology that leverages optimization on global, node, and device levels to achieve unprecedented scalability for tensor networks. This enables the handling of large-scale tensor networks with memory capacities reaching tens of terabytes, surpassing memory space constraints on a single node. Our techniques enable accommodating large-scale tensor networks with up to tens of terabytes of memory, reaching up to 2304 GPUs with a peak computing power of 561 PFLOPS half-precision. Notably, we have achieved a time-to-solution of 14.22 seconds with energy consumption of 2.39 kWh which achieved fidelity of 0.002 and our most remarkable result is a time-to-solution of 17.18 seconds, with energy consumption of only 0.29 kWh which achieved a XEB of 0.002 after post-processing, outperforming Google's quantum processor Sycamore in both speed and energy efficiency, which recorded 600 seconds and 4.3 kWh, respectively.

==> 3_INNOVATIONS/memory/memory.tex <==
\subsection{Memory management}
\label{sec:memory}

During contraction of a tensor network, following parts should be taken into account: two input tensors of contraction, one output of contraction, additional overhead of extra variables and system utilities. To clarify matters, we first categorize network contraction computations into three types. Then, we determine the appropriate memory allocation for each category and subsequently develop memory management strategies.

\subsubsection{Types of contraction}

Stem Type:
We visualize the optimal contraction tree, which consists of a stem path leading from a leaf node to the root node. Nodes on the stem path consume significantly more computation and memory resources than other nodes.
Throughout the tensor network, the stem tensor is present throughout the entire process, and its size typically increases during computations. This type of computation involving stem tensors is referred to as the stem type. 

Split Type:
During the final stages of computation, we apply tensor splitting to the stem tensor. This process involves dividing the stem tensor into smaller chunks, with each chunk performing contraction operations with non-stem chunked inputs. This type of computation involving chunked stem tensors is referred to as the split type.

Common Type:
The computation without the involvement of the stem tensors is called common type. Note: In general, non-stem tensors have manitude of MB.

\subsubsection{Double buffering technique}
A100 has a maximun memory space of 80GB. After accounting for additional overhead of extra variables and system utilities, we are left with 79GB of memory space avaliable for tensors. 
A tensor contraction involve three tensors, input 1, input 2, and output. Since common Type generally involves tensors in the MB range, we simply employ dynamic memory management. 
However, for Stem Type, we have one input and one output being stem tensors, which are of size of $2^n$. To fully utilize the memory space, these tensors can be designed up to 32GB each. To avoid frequent allocation and deallocation of GPU memory, we create two 32GB buffers for stem tensors: one for input and one for output, enabling static memory management.
The double buffer technique can also be applied to Split Type. Instead of occupying two complete and separate buffers, we divide the buffers into contiguous chunks to store the input and output. Note that the unused fragments will not be freed, as we may need to perform multiple subtasks. However, we can manually distribute other temporal variables within these fragments to optimize memory.




==> Makefile <==
base_name := Manuscript
datestamp := $(shell date +"%Y-%m-%d")
workdir   := $(shell basename $(shell pwd))


%.pdf: %.tex
	pdflatex --interaction=nonstopmode $<
	bibtex $*.aux
	pdflatex --interaction=nonstopmode $<
	pdflatex --interaction=nonstopmode $<


all: $(base_name).pdf  
	(evince $(base_name).pdf  &)


$(base_name).pdf: $(base_name).tex $(base_name).bib 

figures:
	$(MAKE) -C figures

dated:
	[ ! -d archive ] && mkdir archive
	$(MAKE) pdf
	cp -a $(base_name).pdf archive/$(base_name)-$(datestamp).pdf

tgz:
	$(MAKE) clean
	cd .. && tar -zcvf $(base_name)-$(datestamp).tgz $(workdir)

backup:
	$(MAKE) tgz
	cd .. && rsync -avizP $(base_name)-$(datestamp).tgz barin:backup/.

semiclean:
	rm -f *~ *.aux *.bbl *.blg *.brf *.bmt *.dvi *.log *.toc \
	$(base_name).pdf $(base_name).ps $(base_name).out $(base_name)Notes.bib

figuresclean:
	$(MAKE) -C figures clean

clean:
	$(MAKE) semiclean

.PHONY: clean figuresclean semiclean backup


==> algo.tex <==
\begin{algorithm}
\LinesNumbered
\label{alg:preprocess}
\KwIn{pauliStrings, n\_qubits}
\KwResult{idxs, pmXY\_buf, pmYZ\_buf, coeffs\_buf}
% \BlankLine

{$N, K \gets n\_qubits, \text{length(pauliStrings)}$\\}
$pmXY, pmYZ \gets \text{zeros}(N,K), \text{zeros}(N,K)$\\

\For{$(i, (coeff, pauliStr))$ \textbf{in} \text{enumerate(pauliStrings)}}{
    $Y_{occ} \gets 0$ \tcp{occurrence for Y}
    \tcc{Construct Pauli mat XY and Pauli mat YZ}
    \For{$(p, pauli)$ \textbf{in} pauliStr}{
        \If{$pauli == "X"$}{
            $pmXY[p, i] \gets 1$\\
        }
        \ElseIf{$pauli == "Y"$}{
            $pmXY[p, i] \gets pmYZ[p, i] \gets 1$\\
            $Y_{occ} \gets Y_{occ} + 1$\\
        }
        \Else{$pmYZ[p, i] \gets 1$}
    }
    \tcc{New coefficients: fuse const calculation}
    $coeff \gets \text{real}(coeff) \times \text{real}((-i)^{Y_{occ}})$ \\

    \tcc{Compressed Pauli mat XY using Dict}
    $sid = \_encode2id(pmXY[:,i])$\\
    \If{\textbf{not} \text{haskey(coeffs\_dict, sid)}}{
        $pmXY\_dict[sid] \gets pmXY[:,i]$\\
    }
    $coeffs\_dict[sid].\text{append}(coeff)$\\
    $pmYZ\_dict[sid].\text{append}([pmYZ[:,i]])$\\
}

\tcc{Compacting data into new continuous buffer}
$L \gets pmXY\_dict.count; idx \gets 0$\\
% $pmXY\_buf, pmYZ\_buf, coeffs\_buf, idxs, idx \gets$ \newline $\text{zeros(N, L)}, \text{zeros(N, K)}, \text{zeros(K)}, \text{zeros(L+1)}, 0$\\

\For{$(i, (sid, pm23))$ \textbf{in} \text{enumerate}(pmYZ\_dict)}{
    $num \gets \text{length}(pm23)$\\
    $pmYZ\_buf[:,idx:idx+num] \gets pm23$ \\
    $pmXY\_buf[:, i] \gets pmXY\_dict[sid]$\\
    $coeffs\_buf[idx:idx+num] \gets coeffs\_dict[sid]$ \\
    $ idx \gets idx + num$; $idxs[i] \gets idx$\\
}

% \Return{$idxs, pmXY\_buf, pmYZ\_buf, coeffs\_buf$}
% \end{algorithmic}
\caption{Preprocess: Hamiltonian data structure optimizations}
\end{algorithm}




\begin{algorithm}
\LinesNumbered
\caption{Calculate Local Energy}
\label{alg:calculate_local_energy}
\KwIn{$\text{idxs}$, $\text{pmXY}$, $\text{pmYZ}$, $\text{coeffs}$, $\text{states}$}

$\text{eloc} \leftarrow 0.0$\\
\For{$\text{state}$ \textbf{in} $\text{states}$}{
    \For{$i \leftarrow 0$ \KwTo $\text{size(pmXY, 2)}$}{
      \tcc{calculate coupled coef}
      $\text{coef} \leftarrow 0.0$\\
      \For{$j \leftarrow \text{idxs}[i]$ \KwTo $\text{idxs}[i+1]$}{
        $\text{tstate} \leftarrow \text{pmYZ}[:, j] \& \text{state}$\\
        $\text{coef} \leftarrow \text{coef} + ((-1)^{\text{cnt\_1}(\text{tstate})}) \times \text{coeffs}[j]$\\
      }
      $\text{cpld\_coefs}[i] \leftarrow \text{coef}$\\
    
      \tcc{calculate coupled states}
      $\text{cpld\_states}[:, i] \leftarrow \text{xor}(\text{state}, \text{pmXY}[:, i])$\\
    }

    \tcc{accumulate local energy of the state}
    $\text{eloc} += \text{dot}(\Psi(\text{cpld\_states}), \text{cpld\_coefs}) / \Psi(\text{state})$\\
}
\KwRet{$\text{eloc}$}\\
\end{algorithm}


\begin{algorithm}
\DontPrintSemicolon
\LinesNumbered
\SetAlgoLined
\KwIn{$n\_qubits$, $NK$, $idxs$, $coeffs$, $pmXY$, $pmYZ$, $batch\_size$, $batch\_size\_cur\_rank$, $ist$, $states$, $id\_lut$, $wf\_lut$}
\KwResult{$res\_elocs$}
\tcc{Initialization of power of two table}
$tbl\_pow2[0...63] \leftarrow \{1, 2,..., 2^{63}\}$ \;
\tcc{Partition for CUDA kernel}
$index \leftarrow blockIdx.x \times blockDim.x + threadIdx.x$ \;
$stride \leftarrow gridDim.x \times blockDim.x$ \;

\For{$ii \leftarrow index$ \KwTo $batch\_size\_cur\_rank$ \textbf{step} $stride$}{
    $eloc\_real, eloc\_imag \leftarrow 0$ \;
    \For{$k \leftarrow 0$ \KwTo $NK$}{
        \tcc{Fuse coupled states and state2id}
        $id \leftarrow 0$ \;
        \For{$j \leftarrow 0$ \KwTo $N$}{
            $id += xor(states[ii \times N+j], pmXY[k \times N+j]) \times tbl\_pow2[j]$ \;
        }
        \tcc{Binary find id among the lookup table}
        $idx \leftarrow binary\_find(id\_lut, id)$ \;
        \If{$idx$ \textbf{does not exist}}{
            \textbf{continue} \;
        }
        \tcc{Calculate coupled coef}
        $coef \leftarrow 0.0$ \;
        \For{$i \leftarrow idxs[k]$ \KwTo $idxs[k+1]$}{
            $sum \leftarrow 0$ \;
            \For{$j \leftarrow 0$ \KwTo $N$}{
                $sum += states[ii \times N+j] \& pmYZ[i \times N+j]$ \;
            }
            $coef += ( (sum \& 1) ? 1 : -1) \times coeffs[i]$ \;
        }
        \tcc{Accumulation}
        $eloc\_real += coef \times wf\_lut[idx \times 2]$ \;
        $eloc\_imag += coef \times wf\_lut[idx \times 2+1]$ \;
    }
    \tcc{Store the result number as return}
    $a, b \leftarrow eloc\_real, eloc\_imag$ \;
    $c, d \leftarrow wf\_lut[(ist+ii) \times 2], wf\_lut[(ist+ii) \times 2+1]$ \;
    $c2\_d2 \leftarrow c^2 + d^2$ \;
    $res\_elocs[ii \times 2] \leftarrow (a \times c + b \times d) / c2\_d2$ \;
    $res\_elocs[ii \times 2+1] \leftarrow -(a \times d - b \times c) / c2\_d2$ \;
}
\caption{Optimizations of local energy calculation}
\end{algorithm}

